Resource-Aware Pareto-Optimal Automated Machine Learning Platform

In this study, we introduce a novel platform Resource-Aware AutoML (RA-AutoML) which enables flexible and generalized algorithms to build machine learning models subjected to multiple objectives, as well as resource and hard-ware constraints. RA-AutoML intelligently conducts Hyper-Parameter Search(HPS) as well as Neural Architecture Search (NAS) to build models optimizing predefined objectives. RA-AutoML is a versatile framework that allows user to prescribe many resource/hardware constraints along with objectives demanded by the problem at hand or business requirements. At its core, RA-AutoML relies on our in-house search-engine algorithm,MOBOGA, which combines a modified constraint-aware Bayesian Optimization and Genetic Algorithm to construct Pareto optimal candidates. Our experiments on CIFAR-10 dataset shows very good accuracy compared to results obtained by state-of-art neural network models, while subjected to resource constraints in the form of model size.

==> RelatedWork.tex <==
\section{Related Work}

Elsken, Metzen, Hutter \cite{JMLR:v20:18-598} laid an architecture for neural architecture search, which contains three parts: search space, search strategy and performance estimation strategy. Search space defines which architecture or hyper-parameters can be represented in the model. Search strategy details how to explore the search space. The performance estimation strategy is the process of estimating model performance, usually refers to high predictive performance on unseen data. A lot of effort is focusing on reducing cost of measuring the performance since it is computationally expensive. We use this framework to define our work space in AutoML as well. 

Another fundamental concept we use to build our workflow on is the building blocks for neural network architectures \cite{DBLP:journals/corr/TargAL16}. Dutta et el.\cite{DBLP:journals/corr/abs-1801-08577} discussed in \textit{Effective Building Block Design for Deep Convolutional Neural Networks using Search} that using building blocks like ResNet block or its variations for neural architecture search achieves high performance of the model and simplifies the search process. Instead of searching for the architecture layer by layer, they use blocks as fundamentals, so now the search space consists of blocks and the search strategy is to find how to optimize the number of blocks. We use this building block idea for our neural architecture workflow, specifically we use ResNet Block for our experiment. 

There are four major search strategies for hyper-parameter tuning. The brute force method is exhaustive search, which includes grid search which performs an exhaustive searching through a manually specified subset of the hyper-parameter space, random search \cite{Bergstra:2012:RSH:2188385.2188395} and batch search, which allows users to simply provide several configurations for the trial code.

The second category is heuristic search, methods like naive evolution \cite{DBLP:journals/corr/RealMSSSLK17}, anneal and hyperband \cite{DBLP:journals/corr/LiJDRT16} belong to this category. Naive evolution randomly initializes a population-based search space. For each generation, it chooses better ones and does some mutation on them to get the next generation. Hyper-band tries to use the limited resource to explore as many configurations as possible, and finds out the promising ones to get the final result.  

Bayesian optimization is a big category by itself, there are different kinds of variations under the general method, for instance, Bayesian Optimization Hyper-band (BOHB) which combines Bayesian optimization with heuristic search hyper-band \cite{DBLP:journals/corr/abs-1807-01774}, Tree-structured Parzen Estimator (TPE) \cite{NIPS2011_4443}, Sequential Model-based Algorithm Configuration (SMAC) \cite{HutHooLey11-smac}, Metis Tuner \cite{li2018metis}, Sequential model-based optimization (SMBO) approach as a tuner with Gaussian Process is often used as surrogate \cite{NIPS2011_4443}, etc. Another big family is reinforcement learning, proximal policy optimization (PPO) algorithms \cite{DBLP:journals/corr/SchulmanWDRK17} is often used as RL tuner for hyper-parameters. 

There are only a few work that are in the budget constraint hyper-parameter tuning field. For instance, Lu, Chiang and Sha \cite{DBLP:journals/corr/abs-1902-00532} proposed to solve single objective hyper-parameter tuning under budget constraint as a sequential decision making problem, such that they can use the partial training progress of configurations to dynamically allocate the remaining budget. Their algorithm combines a Bayesian belief model which estimates the future performance of configurations, with an action-value function which balances exploration-exploitation trade-off, to optimize the final output.

When it comes to training neural networks under multiple objectives, the Pareto method is often used \cite{doi:10.1080/23311916.2018.1502242}. The Pareto method keeps the elements of the solution vector space during optimization and differentiate the dominated and non-dominated solutions. 
Smithson, Yang, Gross, and Meyer \cite{DBLP:journals/corr/SmithsonYGM16} uses neural networks to predict future candidate networks with different hyper-parameters configurations, optimizing for both accuracy and computational complexity, their simulation results approximate the Pareto-optimal front, while only exploring a small fraction of the design space. 

The area that requires multi-objective hyper-parameter tuning under budget constraint remains unexplored. We use the search space, search strategy, model performance framework as a basis, and explores how we can realize the unexplored field.



